Quantifying Inefficiency of Fair Cost-Sharing Mechanisms for Sharing Economy

Sharing economy is a distributed peer-to-peer economic paradigm, which gives rise to a variety of social interactions for economic purposes. One fundamental distributed decision-making process is coalition formation for sharing certain replaceable resources collaboratively, for example, sharing hotel rooms among travelers, sharing taxi-rides among passengers, and sharing regular passes among users. Motivated by the applications of sharing economy, this paper studies a coalition formation game subject to the capacity of $K$ participants per coalition. The participants in each coalition are supposed to split the associated cost according to a given cost-sharing mechanism. A stable coalition structure is established when no group of participants can opt out to form another coalition that leads to lower individual payments. We quantify the inefficiency of distributed decision-making processes under a cost-sharing mechanism by the strong price of anarchy (SPoA), comparing a worst-case stable coalition structure and a social optimum. In particular, we derive SPoA for common fair cost-sharing mechanisms (e.g., equal-split, proportional-split, egalitarian and Nash bargaining solutions of bargaining games, and usage based cost-sharing). We show that the SPoA for equal-split, proportional-split, and usage based cost-sharing (under certain conditions) is $\Theta(\log K)$, whereas the one for egalitarian and Nash bargaining solutions is $O(\sqrt{K} \log K)$. Therefore, distributed decision-making processes under common fair cost-sharing mechanisms induce only moderate inefficiency.

==> append3.tex <==



\begin{customlemma}{11} \label{lem:cyc}
If there exists no cyclic preference, there always exists a stable coalition structure. Furthermore, such a stable coalition structure can be found in time $n^{O(K)}$.
\end{customlemma}


\begin{proof}
%It follows from the fact that if there exists no cyclic preference, then no blocking coalition can exist.
We include the standard argument for completeness (see, e.g., \cite{HVW15} for dynamic coalition formation by local improvements). Consider a directed graph $\cG=(\cN_K,E)$ on the set $\cN_K\triangleq\{S\in 2^\cN:|S|\le K\}$ of subsets of size at most $K$. For two sets $G_1,G_2\in\cN_K$, we define an edge $(G_1,G_2)\in E$ if and only if there is a participant $i\in G_1\cap G_2$ such that $u_i(G_1)<u_i(G_2)$. Then the existence of a cyclic preference is equivalent to the existence of a directed cycle in $\cG$. Thus if there exists no cyclic preference, then $\cG$ is acyclic and hence has at least one sink. 

Let $\cP$ be a maximal subset of sinks in $\cG$ with the property that any two distinct nodes $G,G'\in\cP$ are pairwise disjoint. 
Let $S$ be the set of participants covered by $\cP$, and $\cG'$ be the subgraph of $\cG$ obtained by deleting all the nodes containing some participant in $S$. 

By induction, there is a stable coalition structure $\cP'$ among the set of participants $S'\triangleq\cN\backslash S$. It follows that $\cP\cup\cP'$ is a stable coalition structure on the set of all participants. Indeed, if there is a blocking coalition $G_1$ then $G_1\cap S\neq\varnothing$ (since otherwise $\cP'$ is not stable among the participants in $S'$). But then there must exist $i\in S$ such that contain $u_i(G_1)>u_i(G_2)$, where $G_2\in\cP$ is the coalition containing $i$. This would imply that $(G_2,G_1)\in E$ contradicting that $G_2$ is a sink in $\cG$.  
%\footnote{Note that this is not necessarily true if we use the weaker definition of blocking coalition $G$ by which the utilities of all participants in $G$ do not decrease and the utility of at least one participant strictly increases.}     
\end{proof}

\begin{customthm}{7} 
For equal-split cost-sharing, there always exists a stable coalition structure.
\end{customthm}
\begin{proof}
If there exists a cyclic preference, defined by $(i_1,..., i_s)$ and $(G_1,..., G_s)$, then
\begin{eqnarray*}
u_{i_1}(p^{\rm eq}_{i_1}(G_1)) = c_{i_1} - \frac{c(G_1)}{|G_1|} & > & c_{i_1} - \frac{c(G_2)}{|G_2|} = u_{i_1}(p^{\rm eq}_{i_1}(G_2)), \\
u_{i_2}(p^{\rm eq}_{i_2}(G_2)) = c_{i_2} - \frac{c(G_2)}{|G_2|} & > & c_{i_2} - \frac{c(G_3)}{|G_3|} = u_{i_2}(p^{\rm eq}_{i_2}(G_3)), \\
& \vdots & \notag \\
u_{i_s}(p^{\rm eq}_{i_s}(G_s)) = c_{i_s} - \frac{c(G_s)}{|G_s|} & > & c_{i_s} - \frac{c(G_1)}{|G_1|} = u_{i_s}(p^{\rm eq}_{i_s}(G_1))
\end{eqnarray*}
Summing the above equations, one obtains a contradiction $ 0 > 0$. This completes the proof by Lemma~\ref{lem:cyc}.
\end{proof}

\begin{customthm}{8}
For proportional-split cost-sharing, there always exists a stable coalition structure.
\end{customthm}
\begin{proof}
If $u_{i}(p^{\rm pp}_{i}(G_1)) > u_{i}(p^{\rm pp}_{i}(G_2))$, then
\begin{equation}
c_i - \frac{c_i \cdot c(G_1)}{\sum_{j \in G_1} c_j} > c_i - \frac{c_i \cdot c(G_2)}{\sum_{j \in G_2} c_j} \quad \Rightarrow \quad 
\frac{ c(G_1)}{\sum_{j \in G_1} c_j} < \frac{ c(G_2)}{\sum_{j \in G_2} c_j}
\end{equation}
Thus, if there exists a cyclic preference, then
\begin{equation}
\frac{ c(G_1)}{\sum_{j \in G_1} c_j} < \frac{ c(G_2)}{\sum_{j \in G_2} c_j}<\cdots < \frac{ c(G_s)}{\sum_{j \in G_s} c_j}<\frac{ c(G_1)}{\sum_{j \in G_1} c_j}
\end{equation}
Summing the above equations, one obtains a contradiction $ 0 > 0$. This completes the proof by Lemma~\ref{lem:cyc}.
\end{proof}



\begin{customthm}{9} \label{thm:eqaexist}
For egalitarian cost-sharing, there always exists a stable coalition structure.
\end{customthm}
\begin{proof}
If there exists a cyclic preference, then
\begin{eqnarray}
u_{i_1}(p^{\rm ega}_{i_1}(G_1)) = \frac{(\sum_{j \in G_1} c_j) - c(G_1)}{|G_1|} & > & \frac{(\sum_{j \in G_2} c_j) - c(G_2)}{|G_2|} = u_{i_1}(p^{\rm ega}_{i_1}(G_2)), \\
u_{i_2}(p^{\rm ega}_{i_2}(G_2)) = \frac{(\sum_{j \in G_2} c_j) - c(G_2)}{|G_2|} & > & \frac{(\sum_{j \in G_3} c_j) - c(G_3)}{|G_3|} = u_{i_2}(p^{\rm ega}_{i_2}(G_3)), \\
& \vdots & \notag \\
u_{i_s}(p^{\rm ega}_{i_s}(G_s)) = \frac{(\sum_{j \in G_s} c_j) - c(G_s)}{|G_s|} & > & \frac{(\sum_{j \in G_1} c_j) - c(G_1)}{|G_1|} = u_{i_s}(p^{\rm ega}_{i_s}(G_1))
\end{eqnarray}
Summing the above equations, one obtains a contradiction $ 0 > 0$. This completes the proof by Lemma~\ref{lem:cyc}.
\end{proof}

\iffalse
\begin{customcor}{1} \label{cor:nashir}
If sub-additivity is satisfied, then Nash bargaining solution, irrespective of the constraint of non-negative payments, satisfies individual rationality.
\end{customcor}
\begin{proof}
First, the constraint of non-negative payments is not considered. Then, individual rationality follows from Lemma~\ref{lem:eqanash} and the fact that egalitarian cost-sharing satisfies individual rationality, when sub-additivity is satisfied.

Second, the constraint of non-negative payments is considered. Let $H \subseteq G$ be the set of participants with positive payment in $G$, such that $p^{\rm nash}_{i}(G) > 0$ for $i \in H$. By Lemma~\ref{lem:nash2}, it suffices to show that $p^{\rm nash}_{i}(G) \le c_i$, namely, $(\sum_{j \in H} c_j) - c(G) \ge 0$. Note that if $k \not\in H$, then by Lemma~\ref{lem:nash2},
\begin{equation}
0 \le c_k \le \frac{(\sum_{j \in H} c_j) - c(G)}{|H|}
\end{equation}
This completes the proof.
\end{proof}
\fi

==> usage-ex.tex <==


\section{Example of Usage Based Cost Sharing} \label{sec:usage-ex}

\begin{table}[htb!]
{\scriptsize
\begin{equation*}
\begin{array}{rl}
(\textsc{P1}) \ \max & X_1(\{1\})+\frac{X_1(\{1,2\})}{2}+\frac{X_1(\{1,3\})}{2}+\frac{X_1(\{1,2,3\})}{3}+X_2(\{2\})+\frac{X_2(\{2,3\})}{2}+X_3(\{3\})\\
\text{subject to} &\\
{\lambda(\{2,3\},1,2)}:&  X_2(\{2\})+X_2(\{3\})+X_2(\{2,3\}) \le  X_1(\{2\})+X_1(\{3\})+X_1(\{1,2\})+X_1(\{1,3\})+ X_1(\{2,3\})+X_1(\{1,2,3\})\\
{\lambda(\{3\},1,3)}:&X_3(\{3\})\le X_1(\{3\})+X_1(\{1,3\}) + X_1(\{2,3\})+X_1(\{1,2,3\})  \\
{\lambda(\{3\},2,3)}:&X_3(\{3\})\le X_2(\{3\})+ X_2(\{2,3\})  \\
{z}:& X_1(\{1\})+X_1(\{2\})+X_1(\{3\})+X_1(\{1,2\})+X_1(\{1,3\})+ X_1(\{2,3\})+X_1(\{1,2,3\})\le 1\\
&X_1(\{1\}),X_1(\{2\}),X_1(\{3\}),X_1(\{1,2\}),X_1(\{1,3\}),X_1(\{2,3\})\ge 0,\\
&X_1(\{1,2,3\}),X_2(\{2\}),X_2(\{3\}),X_2(\{2,3\}),X_3(\{3\})\ge  0.
\end{array}
\end{equation*}
}
{\scriptsize
\begin{equation*}
\begin{array}{rl}
(\textsc{D1}) \ \min &  z\\
\text{subject to} &\\
{X_2(\{2\})}: & \lambda(\{2,3\},1,2) \ge  1 \\
{X_2(\{3\})}: & \lambda(\{2,3\},1,2)-\lambda(\{3\},2,3) \ge  0 \\
{X_2(\{2,3\})}:  & \lambda(\{2,3\},1,2)-\lambda(\{3\},2,3) \ge \frac{1}{2} \\
{X_3(\{3\})}: &\lambda(\{3\},1,3)+\lambda(\{3\},2,3) \ge  1\\
{X_1(\{1\})}: &1\le z\\
{X_1(\{2\})}: & \lambda(\{2,3\},1,2)\le z\\
{X_1(\{3\})}: &\lambda(\{2,3\},1,2) + \lambda(\{3\},1,3)\le z\\
{X_1(\{1,2\})}:&\frac{1}{2}+  \lambda(\{2,3\},1,2)\le z\\
{X_1(\{1,3\})}: &\frac{1}{2}+  \lambda(\{2,3\},1,2)+\lambda(\{3\},1,3)\le z\\
{X_1(\{2,3\})}: & \lambda(\{2,3\},1,2)+ \lambda(\{3\},1,3)\le z\\
{X_1(\{1,2,3\})}: &\frac{1}{3}+ \lambda(\{2,3\},1,2)+ \lambda(\{3\},1,3)\le z\\
& \lambda(\{2,3\},1,2),\lambda(\{3\},1,3),\lambda(\{3\},2,3)\ge 0
\end{array}
\end{equation*}
}
{\scriptsize
\begin{equation*}
\begin{array}{rl}
(\textsc{D2}) \ \min & \lambda(\{2,3\},1,2)+\lambda(\{3\},1,3)+\lambda(\{3\},2,3)\\
\text{subject to} &\\
{X_2(\{2\})}: & \lambda(\{2,3\},1,2)=  1 \\
{X_2(\{3\})}: & \lambda(\{2,3\},1,2)-\lambda(\{3\},2,3)=  0 \\
{X_2(\{2,3\})}:  & \lambda(\{2,3\},1,2)-\lambda(\{3\},2,3) = \frac{1}{2} \\
{X_3(\{3\})}: &\lambda(\{3\},1,3)+\lambda(\{3\},2,3) =  1\\
& \lambda(\{2,3\},1,2),\lambda(\{3\},1,3),\lambda(\{3\},2,3)\ge 0
\end{array}
\end{equation*}
}
{\scriptsize
\begin{equation*}
\begin{array}{rl}
(\textsc{P2}) \ \max &  X_1(\{1\})+\frac{X_1(\{1,2\})}{2}+\frac{X_1(\{1,2,3\})}{3}+X_2(\{2\})+\frac{X_2(\{2,3\})}{2}+X_3(\{3\})\\
\text{subject to} &\\
{\lambda(\{2,3\},1,2)}:&  X_2(\{2\})+X_2(\{3\})+X_2(\{2,3\}) \le  1\\
{\lambda(\{3\},1,3)}:&X_3(\{3\})\le 1 \\
{\lambda(\{3\},2,3)}:&X_3(\{3\})\le X_2(\{3\})+ X_2(\{2,3\})+1.
\end{array}
\end{equation*}
}
\caption{Example when $K=3$.}
\end{table}


\iffalse
\begin{table}[htb!]
\centering
\caption{Example when $K=3$.}
\label{tab:usage-k3}
\begin{tabular}{ll}
(\textsc{P1}) &  
{\scriptsize
\begin{align}
\max & \quad X_1(\{1\})+\frac{X_1(\{1,2\})}{2}+\frac{X_1(\{1,3\})}{2}+\frac{X_1(\{1,2,3\})}{3}+X_2(\{2\})+\frac{X_2(\{2,3\})}{2}+X_3(\{3\})\\
\text{subject to} &\\
{\lambda(\{2,3\},1,2)}:&  X_2(\{2\})+X_2(\{3\})+X_2(\{2,3\}) \le  X_1(\{2\})+X_1(\{3\})+X_1(\{1,2\})+X_1(\{1,3\})+ X_1(\{2,3\})+X_1(\{1,2,3\})\\
{\lambda(\{3\},1,3)}:&X_3(\{3\})\le X_1(\{3\})+X_1(\{1,3\}) + X_1(\{2,3\})+X_1(\{1,2,3\})  \\
{\lambda(\{3\},2,3)}:&X_3(\{3\})\le X_2(\{3\})+ X_2(\{2,3\})  \\
{z}:& X_1(\{1\})+X_1(\{2\})+X_1(\{3\})+X_1(\{1,2\})+X_1(\{1,3\})+ X_1(\{2,3\})+X_1(\{1,2,3\})\le 1\\
&X_1(\{1\}),X_1(\{2\}),X_1(\{3\}),X_1(\{1,2\}),X_1(\{1,3\}),X_1(\{2,3\})\ge 0,\\
&X_1(\{1,2,3\}),X_2(\{2\}),X_2(\{3\}),X_2(\{2,3\}),X_3(\{3\})\ge  0.
\end{align}
}
\\
(\textsc{D1}) &   
{\scriptsize
\begin{align}
\min & \quad z\\
\text{subject to} &\\
{X_2(\{2\})}: & \lambda(\{2,3\},1,2) \ge  1 \\
{X_2(\{3\})}: & \lambda(\{2,3\},1,2)-\lambda(\{3\},2,3) \ge  0 \\
{X_2(\{2,3\})}:  & \lambda(\{2,3\},1,2)-\lambda(\{3\},2,3) \ge \frac{1}{2} \\
{X_3(\{3\})}: &\lambda(\{3\},1,3)+\lambda(\{3\},2,3) \ge  1\\
{X_1(\{1\})}: &1\le z\\
{X_1(\{2\})}: & \lambda(\{2,3\},1,2)\le z\\
{X_1(\{3\})}: &\lambda(\{2,3\},1,2) + \lambda(\{3\},1,3)\le z\\
{X_1(\{1,2\})}:&\frac{1}{2}+  \lambda(\{2,3\},1,2)\le z\\
{X_1(\{1,3\})}: &\frac{1}{2}+  \lambda(\{2,3\},1,2)+\lambda(\{3\},1,3)\le z\\
{X_1(\{2,3\})}: & \lambda(\{2,3\},1,2)+ \lambda(\{3\},1,3)\le z\\
{X_1(\{1,2,3\})}: &\frac{1}{3}+ \lambda(\{2,3\},1,2)+ \lambda(\{3\},1,3)\le z\\
& \lambda(\{2,3\},1,2),\lambda(\{3\},1,3),\lambda(\{3\},2,3)\ge 0
\end{align}
}
\\
(\textsc{D2}) &     
{\scriptsize
\begin{align}
\min & \quad  \lambda(\{2,3\},1,2)+\lambda(\{3\},1,3)+\lambda(\{3\},2,3)\\
\text{subject to} &\\
{X_2(\{2\})}: & \lambda(\{2,3\},1,2)=  1 \\
{X_2(\{3\})}: & \lambda(\{2,3\},1,2)-\lambda(\{3\},2,3)=  0 \\
{X_2(\{2,3\})}:  & \lambda(\{2,3\},1,2)-\lambda(\{3\},2,3) = \frac{1}{2} \\
{X_3(\{3\})}: &\lambda(\{3\},1,3)+\lambda(\{3\},2,3) =  1\\
& \lambda(\{2,3\},1,2),\lambda(\{3\},1,3),\lambda(\{3\},2,3)\ge 0
\end{align}
}
\\
(\textsc{P2}) & 
{\scriptsize
\begin{align}
\max & \quad X_1(\{1\})+\frac{X_1(\{1,2\})}{2}+\frac{X_1(\{1,2,3\})}{3}+X_2(\{2\})+\frac{X_2(\{2,3\})}{2}+X_3(\{3\})\\
\text{subject to} &\\
{\lambda(\{2,3\},1,2)}:&  X_2(\{2\})+X_2(\{3\})+X_2(\{2,3\}) \le  1\\
{\lambda(\{3\},1,3)}:&X_3(\{3\})\le 1 \\
{\lambda(\{3\},2,3)}:&X_3(\{3\})\le X_2(\{3\})+ X_2(\{2,3\})+1.
\end{align}
}    
\end{tabular}
\end{table}
\fi

